Latent Representation Learning for Multimodal Brain Activity Translation

Neuroscience employs diverse neuroimaging techniques, each offering distinct insights into brain activity, from electrophysiological recordings such as EEG, which have high temporal resolution, to hemodynamic modalities such as fMRI, which have increased spatial precision. However, integrating these heterogeneous data sources remains a challenge, which limits a comprehensive understanding of brain function. We present the Spatiotemporal Alignment of Multimodal Brain Activity (SAMBA) framework, which bridges the spatial and temporal resolution gaps across modalities by learning a unified latent space free of modality-specific biases. SAMBA introduces a novel attention-based wavelet decomposition for spectral filtering of electrophysiological recordings, graph attention networks to model functional connectivity between functional brain units, and recurrent layers to capture temporal autocorrelations in brain signal. We show that the training of SAMBA, aside from achieving translation, also learns a rich representation of brain information processing. We showcase this classify external stimuli driving brain activity from the representation learned in hidden layers of SAMBA, paving the way for broad downstream applications in neuroscience research and clinical contexts.

==> sections/interpretations.tex <==
\subsection{Interpretation} 
\label{sec:interpretation}

\begin{figure*}[h]
    \centering
    \begin{minipage}[t]{0.30\textwidth}
        \centering
        \vspace{0pt} % Ensures alignment at the top
        \includegraphics[width=\textwidth]{figures/results/reconstructions.pdf}
        \caption{\footnotesize Given MEG data, \model{} reconstructs three minutes of fMRI data per parcel. Ground truth and predictions are color-coded in blue and red, respectively. Each box presents a randomly selected parcel. Except for some parcels like {\tiny Cont\_BPFCmp\_1}, \model{} successfully captures the patterns of the fMRI data using MEG (see supp. mat.).
        }
        \label{fig: reconstruction}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.35\textwidth}
        \centering
        \vspace{0pt} % Ensures alignment at the top
        \includegraphics[width=\textwidth]{figures/results/interperations_hrf.pdf}
        \caption{\footnotesize Inferred undershoot and response dispersion parameters shown in the first and second rows. Parameters smoothly vary across brain regions (x-axis). A) reveals that averaging across subjects results in HRFs that vary by parcel. HRF shapes in different cortical lobes such as occipital, parietal, and temporal (see supp. mat.).} 
        \label{fig: hrf_params}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.30\textwidth}
        \centering
        \vspace{0pt} % Ensures alignment at the top
        \includegraphics[width=\textwidth]{figures/results/wavelet_attentions.pdf}
        \caption{\footnotesize Wavelet decomposition attention and reconstruction loss dynamics. A shows a heatmap over randomly selected brain parcels, with lower frequencies having higher attention weights. B shows overall attention averaged across parcels for each band. C presents the skip loss dynamics (see supp. mat.).}
        \label{fig:wavlet_attention}
    \end{minipage}
     % \vspace{-8pt} 
\end{figure*}




Our model also offers neuroscientific interpretations on different levels. Here, we outline key findings from the best MEG-to-fMRI performing model.

\paragraph{Learned HRFs reveal variable neurovascular coupling across brain regions} 
The first stage of our model's electrophysiological-to-hemodynamic mapping involves parameterized HRF learning. Fig.~\ref{fig: hrf_params} displays the inferred HRF parameters for each brain parcel across subjects. Fig.~\ref{fig: hrf_params} A shows the variation in HRF response and undershoot dispersion across different brain regions, highlighting the diversity in oxygenation and deoxygenation levels~\cite{herculano2009human}. Notably, the left somatomotor network exhibits minimal response dispersion compared to the cingulate, whereas the parietal lobe regions show greater undershoot dispersion than the regions in right somatomotor network. Despite averaging these parameters across subjects, Fig.~\ref{fig: hrf_params} C reveals distinct HRF shapes across the occipital, parietal, and temporal lobes. See the supplementary materials for additional results.


 
 
\paragraph{SAMBA attends to lower frequencies in wavelet denoising} Fig.~\ref{fig:wavlet_attention} illustrates the dynamics of wavelet decomposition attention and wavelet reconstruction skip loss in our model. Specifically, Fig.~\ref{fig:wavlet_attention} A presents a heatmap of variations in randomly selected brain regions, with an average across all parcels shown in Fig.~\ref{fig:wavlet_attention} B. Our model predominantly focuses on lower frequencies, likely due to the higher signal-to-noise ratio at these frequencies compared to higher frequencies. Additionally, Fig.~\ref{fig:wavlet_attention} C details the loss dynamics during wavelet reconstruction. 

 

 
\paragraph{SAMBA infers connectivity via graph attention} Fig.~\ref{fig: graph_interpretations} presents graph interpretations on both brain regions with circular plots at A and B and in parcel level at C. The circular plots in A present how \model{} infers different attention across various regions of the brain in both the left hemisphere (LH) and right hemisphere (RH). For better visualization, we have removed the self-parcel attention, while presenting the second top attention between regions. Though both hemispheres show similar patterns, \model{} infers some differences. For example, saliency/ventral attention network attends to the visual cortex in RH, which is missed in LH (shown by the arrow). Additionally, there is a difference in the attention connectivity between auditory cortex and other brain regions. B presents how different brain regions on the top row's nodes help to reconstruct the bottom nodes in the LH, and the width of the blue lines shows the attention weights. As presented, the visual cortex plays a major role in reconstructing the default mode network. C presents the biclustered attention weights across all of the brain parcels. For example, the AudTemporal parcel presents similar and higher attention patterns with some visual and dorsal attention regions, shown in the bottom right of the figure. 


\begin{figure} %[h]
    \centering
    \includegraphics[width=\textwidth]{figures/results/interperations_graph.pdf}
    \caption{\footnotesize Graph attention visualization: A)  Across brain regions in the left (LH) and right hemispheres (RH), key differences are highlighted by dark arrows on the outer ring. B) Bipartite visualization highlights how upper nodes assist lower nodes, with edge width indicating attention strength; self-parcel attention is omitted for clarity. C) Biclustered attention matrix, with lower left and upper left revealing relationships within the visual cortex. }
    \label{fig: graph_interpretations}
\end{figure}









\input{tables/ablations}

 


\subsection{Classification and ablations} 
We enhanced \model{} with a classification head to identify eight distinct movies from the Naturalistic Viewing dataset~\cite{telesford2023open}. Table~\ref{tab: classification} compares our model's performance against baseline methods. Notably, our model achieves a 7.87\% improvement in EEG to fMRI matching tasks over the baseline. For more details, see the supp. mat. Removing the classification head and visualizing the embedding space of \model{}, (Fig.~\ref{fig: phate_visualization}) reveals that our model effectively clusters samples, indicating that SAMBA can be used as a pre-trained model for other downstream tasks. We used the PHATE~\cite{moon2019visualizing} for visualization, which captures local and global structures in high-dimensional data, effectively revealing meaningful patterns.



 

==> sections/problem_setup.tex <==
\section{Problem Setup}
\label{sec:problem_setup}


Consider the task of translating between electrophysiological and hemodynamic measurements of brain activity. Let $\mathcal{X} = \{\mathbf{x}_1, \mathbf{x}_2, \ldots, \mathbf{x}_{\text{N}}\}$ represent measurements from \(\text{N}\) different brain regions obtained using an electrophysiological technique like EEG or MEG with high temporal sampling rate. 

Concurrently, let $\mathcal{Y} = \{\mathbf{y}_1, \mathbf{y}_2, \ldots, \mathbf{y}_{\text{M}}\}$ denote hemodynamic measurements, captured from $\text{M}$ distinct physiological regions, offering a detailed spatial map of brain activity. Typically, $\text{M} >> \text{N}$, illustrating the superior spatial resolution of hemodynamic modalities that encompass more regions than their electrophysiological counterparts.
Here, we conceptualize physiological regions as distinct, spatially contiguous parcels, as defined in the Schaefer brain atlas~\cite{schaefer2018local}. Given the inherent trade-offs between spatial and temporal resolutions in these modalities, we define the task of bidirectional translation between the two spatiotemporal domains, \(\mathcal{X}\) and \(\mathcal{Y}\). Our goal is to facilitate cross-modal integration, allowing for comprehensive analyses that leverage the strengths of both modalities. This translation aims to address the discrepancies in spatial and temporal resolutions, enabling rich insights from joint modal interpretations.













































% \begin{wrapfigure}[21]{r}{0.29\textwidth}
%     \centering
%     \begin{minipage}[t]{\textwidth}
%         \centering
%         \includegraphics[width=0.29\textwidth]{figures/schematics/problem_setup.pdf}
%         \subcaption[width=0.29\textwidth]{\footnotesize Interlinking electrophysiological \(\mathcal{X}\) data (characterized by high temporal but low spatial resolution), with hemodynamic \(\mathcal{Y}\) data (noted for its high spatial but low temporal resolution) also on the gray-shaded side. The task is to perform spatial and temporal alignment between both modalities.}
%         \label{fig:prob_setup}
%     \end{minipage}
%     \vspace{5mm} % Adjust the space between the subfigures as needed

%     \begin{minipage}[t]{\textwidth}
%         \centering
%         \includegraphics[width=0.29\textwidth]{figures/schematics/framework.pdf} % Replace with your actual file name
%         \subcaption{\footnotesize  Our \model{} as a translation model between electrophysiological ($\mathcal{X}$) and hemodynamic ($\mathcal{Y}$) modalities, derived from same stimuli. } 
%         \label{fig:overview}
%     \end{minipage}
%     \caption{\footnotesize Overall figure caption goes here.}
%     \label{fig:overall}
% \end{wrapfigure}
% \begin{wrapfigure}[21]{r}{0.29\textwidth}
%     \centering
%     \begin{minipage}[t]{\textwidth}
%         \centering
%         \includegraphics[width=0.29\textwidth]{figures/schematics/problem_setup.pdf}
%         \subcaption{\footnotesize Interlinking electrophysiological \(\mathcal{X}\) data (characterized by high temporal but low spatial resolution), with hemodynamic \(\mathcal{Y}\) data (noted for its high spatial but low temporal resolution) also on the gray-shaded side. The task is to perform spatial and temporal alignment between both modalities.}
%         \label{fig:prob_setup}
%     \end{minipage}
%     \vspace{5mm} % Adjust the space between the subfigures as needed
%     \begin{minipage}[t]{\textwidth}
%         \centering
%         \includegraphics[width=0.29\textwidth]{figures/schematics/framework.pdf} % Replace with your actual file name
%         \subcaption{\footnotesize Another figure caption goes here.}
%         \label{fig:overview}
%     \end{minipage}
%     \caption{Overall figure caption goes here.}
%     \label{fig:overall}
% \end{wrapfigure}

%Fig.~\ref{fig:prob_setup} depicts the problem setup of facilitating spatial and temporal translations between electrophysiological techniques (e.g. EEG) and hemodynamic methods (e.g. fMRI). Let \(\mathcal{X} = \{\mathbf{x}_1, \mathbf{x}_2, \ldots, \mathbf{x}_{\text{N}}\}\) be the assembled collection of electrophysiological recordings, encapsulating the neural activity within  \(\text{N}\) different regions. Concurrently, denote \(\mathcal{Y} = \{\mathbf{y}_1, \mathbf{y}_2, \ldots, \mathbf{y}_{\text{M}}\}\) be the corresponding set of hemodynamic recordings that capture the nuanced dynamics across \(\text{M}\) distinct neural physiological regions. In this setting, on one hand, \(\text{M}>\text{N}\) underscores the fact that hemodynamic modalities, with their superior spatial resolution, provide a detailed view of brain activity in more spatial regions than electrophysiological modalities, offering a complementary perspective. On the other hand, electrophysiological methods offer high temporal resolutions compared to hemodynamic data modalities. In this work, we consider physiological regions as distinct parcels located within the gray matter, characterized by their spatial contiguity known as Schaefer brain atlas~\cite{schaefer2018local}. Given the discussed space-time trade-offs, we now define the task of bidirectional translation between two spatiotemporal discrepancy domains $\mathcal{X}$ and $\mathcal{Y}$ to facilitate cross-modal integration, with both modalities derived from the same simulations. 



==> sections/related_works.tex <==
\section{Related works}\label{sec:related}
 

Research in multi-modal neuroimaging synthesis and analysis has advanced significantly, showcasing unique contributions to translating brain activity. The \textit{classical-based} approach laid the foundational understanding for synthesizing fMRI data from EEG signals, introducing both comprehensive theoretical frameworks and practical tools for multi-modal synthesis~\cite{calhas2020eeg, calhas2023eeg, sirpal2022multimodal}. These initial efforts established the groundwork for more sophisticated analyses and synthesis between EEG and fMRI data. In the \textit{ConvNet-based} approach, the focus shifted towards leveraging convolutional neural networks to enrich the analysis of fMRI data with information derived from EEG recordings. This marked a substantial progression in the integrated interpretation of concurrent EEG-fMRI datasets~\cite{abreu2018eeg, liu2019convolutional}.
Unlike classic and ConvNet methods, our model generalizes the multi-modal brain signal translation from electrophysiological to hemodynamic and vice versa. 

==> tables/classification_comparision.tex <==
\begin{table}[ht]
\centering
\captionsetup{width=0.5\textwidth}
\caption{\footnotesize Classification evaluations of SAMBA using EEG-fMRI dataset. \arman{woking on this part}}
\resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{rl!{\vrule}cc}
        \toprule       
        &              
        & EEG-to-fMRI & fMRI-to-EEG   
         \\   
        \cmidrule(lr){1-4}    
         & 1D-CNN 
         & 48.83\tperc   & 30.69\tperc      
         \\   
         & LSTM 
         & 53.71\tperc   & 37.09\tperc      
         \\   
         & Transformer
         & 51.04\tperc   & 38.24\tperc        
         \\*[.5em]
         & SAMBA
         & \textbf{61.28}\tperc  & \textbf{46.50}\tperc              
          \\*[.25em]        
        \bottomrule  
    \end{tabular}
}
\label{tab: classfication}
\end{table}


 
